Supervisor Localization of Discrete-Event Systems under Partial Observation

Recently we developed supervisor localization, a top-down approach to distributed control of discrete-event systems. Its essence is the allocation of monolithic (global) control action among the local control strategies of individual agents. In this paper, we extend supervisor localization by considering partial observation; namely not all events are observable. Specifically, we employ the recently proposed concept of relative observability to compute a partial-observation monolithic supervisor, and then design a suitable localization procedure to decompose the supervisor into a set of local controllers. In the resulting local controllers, only observable events can cause state change. Further, to deal with large-scale systems, we combine the partial-observation supervisor localization with an efficient architectural synthesis approach: first compute a heterarchical array of partial-observation decentralized supervisors and coordinators, and then localize each of these supervisors/coordinators into local controllers.

==> Subsec_RobustControl.tex <==

%\subsection{Robust Supervisory Control Subject to Intermittent Loss of Observations}

In the previous sections, we have assumed that the observable events
can \emph{always} be observed. In this section we consider further
that some observable events are subject to \emph{intermittent loss};
that is, observation of these events may sometimes get lost, due to
for example unreliable sensors.

For the setting of intermittent observation loss, several approaches
have been proposed \cite{XuKumar:2009,UshioTakai:2009,AlvesEt:2014,AlvesEt:2015}
to the corresponding supervisor synthesis. Here we adopt the
approach of \cite{AlvesEt:2015}, for the reason that relative
observability is used in the supervisor design. In particular, we
will use the method in \cite{AlvesEt:2015} to compute a \emph{robust
supervisor} against intermittent observation loss, and then apply
the developed partially-observed supervisor localization to
decompose the robust supervisor into a set of local controllers. In
this way, the resulting local controllers are also robust against
intermittent observation loss.

%[AlvesEt:2014: authors, title, submitted for publication. Also see
%(conference paper information)]

Again let ${\bf G} = (Q,\Sigma, \delta, q_0, Q_m)$ as in
(\ref{eq:plant}) be the plant, and $\Sigma_{o} \subseteq \Sigma$ the
observable event set. To model intermittent loss of observation, let
\[\Sigma_o = \Sigma_{l} \ \dot\cup \ \Sigma_{ul}\]
where $\Sigma_{l}$ denotes the subset of observable events subject
to intermittent loss, while $\Sigma_{ul}$ the subset not subject to
intermittent loss. For each event $\sigma \in \Sigma_{l}$, create a
new event $\sigma'$ which means that observation of $\sigma$ is
lost. Let $\Sigma_{l}' := \{\sigma'| \sigma \in \Sigma_{l}\}$,
$\Sigma' := \Sigma \cup \Sigma_{l}'$, and define the \emph{dilation}
mapping $D:\Sigma^* \rightarrow Pwr(\Sigma')^*$ as follows:
\begin{equation} \label{eq:dilation}
\begin{split}
\mbox{(i)}~&D(\epsilon) = \epsilon; \\
\mbox{(ii)}~&D(\sigma) = \left\{
  \begin{array}{ll}
    \sigma, & \hbox{if $\sigma \notin \Sigma_{l}$,} \\
    \{\sigma,\sigma'\}, & \hbox{if $\sigma \in \Sigma_{l}$;}
  \end{array}
\right.\\
\mbox{(iii)}~&D(s\sigma) = D(s)D(\sigma),\ \ s \in \Sigma^*, \sigma
\in \Sigma.
\end{split}
\end{equation}
Extend $D$ to $D : Pwr(\Sigma)^* \rightarrow Pwr(\Sigma')^*$.

The dilation of plant $G$ is the generator
\begin{align} \label{eq:dilplant}
{\bf G}' = (Q, \Sigma', \delta', q_0, Q_m)
\end{align}
formed by adding to each transition of $G$ labeled with event
$\sigma \in \Sigma_l$ a parallel transition labeled with $\sigma'
\in \Sigma'_l$. Thus the transition function $\delta': Q \times
\Sigma' \rightarrow Q$ is given by
\begin{align*}
(\forall q \in Q, \forall \sigma \in \Sigma)\ \delta(q,\sigma)!
\Rightarrow &(\forall \sigma_l \in D(\sigma))~\\
&[(\delta'(q,\sigma_l)!
\ \&\ \delta'(q,\sigma_l) = \delta(q,\sigma) ]
\end{align*}
According to \cite{AlvesEt:2015}, the closed and marked behaviors of
the dilated plant ${\bf G}'$ are $L({\bf G}') = D(L({\bf G}))$ and
$L_m({\bf G}') = D(L_m({\bf G}))$.

Now let $E \subseteq \Sigma$ be a specification language, and define
\begin{align*}
K := \sup\mathcal{CO}(E \cap L_m({\bf G})).
\end{align*}
Then $K \subseteq L_m({\bf G})$ is controllable (wrt. ${\bf G}$ and
$\Sigma_{uc}$) and observable (wrt. ${\bf G}$ and $P:\Sigma^*
\rightarrow \Sigma^*_o$). Moreover $D(K) \subseteq D(L_m({\bf G})) =
L_m({\bf G}')$. Let $\Sigma'_{uc} := \{\sigma' | \sigma \in \Sigma_l
\cap \Sigma_{uc}\}$, $P' : (\Sigma')^* \rightarrow \Sigma^*_o$, and
define
\begin{align*}
\mathcal{CO}(D(K)) = &\{K' \subseteq D(K) \ | \\
& \hbox{$K'$ is controllable wrt. ${\bf G}'$ and $\Sigma_{uc} \cup \Sigma'_{uc}$}\\
& \&\ \hbox{$K'$ is $D(K)$-observable wrt. ${\bf G}'$ and $P'$} \}
\end{align*}
Then $\mathcal{CO}(D(K))$ is nonempty (the empty language belongs)
and is closed under set union. Therefore the supremal element
$\sup\mathcal{CO}(D(K))$ and may be effectively computed [3]. It is
shown in \cite{AlvesEt:2014} that a supervisor ${\bf RSUP}$ with
\begin{align} \label{eq:rob_monoSUP}
L_m({\bf RSUP}) = \sup\mathcal{CO}(D(K))
\end{align}
is robust against intermittent loss of observing events in
$\Sigma_l$.

Having obtained the robust supervisor ${\bf RSUP}$, we apply the
partially-observed localization procedure to decompose ${\bf RSUP}$
into a set of local controllers ${\bf RLOC}_{\alpha}$, one for each
controllable event $\alpha \in \Sigma_c$. By Theorem~\ref{thm:equ},
these local controllers are control equivalent to the monolithic
${\bf RSUP}$, i.e.
\begin{align*}
   L_m({\bf G}') \cap L_m({\bf RLOC}) &= L_m({\bf RSUP}) \\
   L({\bf G}') \cap L({\bf RLOC}) &= L({\bf RSUP}),
\end{align*}
where $L_m({\bf RLOC}) = ||_{\alpha \in \Sigma_{c}} L_m({\bf
RLOC}_{\alpha})$ and $L({\bf RLOC}) = ||_{\alpha \in \Sigma_{c}}
L({\bf RLOC}_{\alpha})$. Therefore the resulting local controllers
collectively achieve the same robust controlled behavior as ${\bf
RSUP}$ against intermittent loss of observing events in $\Sigma_l$.

In the following, we demonstrate the above {\it robust localization}
procedure again on the Transfer Line system $\bf TL$ as displayed in
Fig.~\ref{fig:TL}. The event set of $\bf TL$ is $\Sigma =
\{1,2,3,4,5,6,8\}$. Assume that the set of observable events is
$\Sigma_o = \{1,2,4,5,6,8\}$ (thus $\Sigma_{uo} = \{3\}$), and the
set of observable events subject to intermittent observation loss is
$\Sigma_{l} = \{6\}$ (thus $\Sigma_{ul} = \{1,2,4,5,8\}$). Also we
have $\Sigma_{l}' = \{6'\}$, and $\Sigma' = \Sigma \cup \Sigma'_{l}
= \{1,2,3,4,5,6,8,6'\}$.

With $\Sigma'_{l}$, we first construct the dilated Transfer Line
system ${\bf TL}'$ as in (\ref{eq:dilplant}). The control
specification is again to protect the two buffers against underflow
and overflow. We compute as in (\ref{eq:rob_monoSUP}) a robust
monolithic supervisor ${\bf RSUP}$, which has 39 states. Then we
apply the partially-observed localization algorithm on ${\bf RSUP}$
to get the corresponding local controllers, as displayed in
Fig.~\ref{fig:robustLoc}. It is verified that these local
controllers are control equivalent to the robust monolithic
supervisor ${\bf RSUP}$; therefore their collective behavior is
robust against intermittent loss of observation of event 6.

\begin{figure}[!t]
\centering
    \includegraphics[scale = 0.18]{Figures/TL_Robust_LOC.eps}
\caption{Transfer Line: Robust local controllers with $\Sigma_{ilo} = \{6\}$}
\label{fig:robustLoc}
\end{figure}

%When no loss of observation of event 6, the local controllers
%achieve the same behavior with ${\bf SUP}$; when the observations of
%event 6 are completely lost, the local controllers achieve the same
%behavior with the case $\Sigma_{uo} = \{3, 6\}$; when the
%observations of event 6 are subject to intermittent loss, the
%collective behavior of the local controllers is $L_m({\bf
%SUP}_{rob}) \subseteq D(L_m({\bf SUP}))$.

Inspecting the transition diagrams of the robust local controllers
displayed in Fig.~\ref{fig:robustLoc}, only ${\bf RLOC}_1$ needs to
observe event 6, and hence the intermittent loss of observation of 6
affects only the control logic of ${\bf RLOC}_1$. The control logic
of ${\bf RLOC}_1$ is to ensure that no more than three workpieces
can be processed in the material-feedback loop, which can be
realized by counting the occurrences of event 2 (input a workpiece
into the loop) and event 6 (output a workpiece from the loop). When
event 6 is observed, it is directly counted and the total number of
workpieces in the loop is decreased by 1 (as in the full observation
case). On the other hand, when event 6 is not observed, the events 5
and 8 instead must be counted so as to infer the occurrence of 6 (as
in the case $\Sigma_{uo} = \{3,6\}$ presented in Section IV).
Finally note that in the transition diagram of ${\bf RLOC}_1$, the
selfloop of event $6'$ means that at the corresponding states, the
occurrence of event 6 is not observed by ${\bf RLOC}_1$; on the
other hand, the transitions labeled with event 6 mean that the
occurrence of event $6$ is observed.





%%% the end%%

